Compliance, Capability, and Conflict: Benchmarking Multimodal LLMs under System Messages

Production deployments of Multimodal Large Language Models (MLLMs) increasingly rely on system messages to govern model behavior. Yet existing benchmarks either evaluate constraints in text only or embed them into the user turn, leaving system-message adherence in multimodal contexts largely unmeasured; they also leave open whether compliance comes at the cost of foundational vision-language capabilities. We introduce VSysBench, a benchmark built on MMVet-v2 that organizes constraints into 5 main categories and 22 sub-categories, ranging from textual directives in visual contexts to fully vision-grounded ones, each paired with a misaligned counterpart that stress-tests the instructional hierarchy. VSysBench scores each response jointly along two axes, constraint compliance and answer correctness, via the Joint Satisfaction Rate (JSR) and Cross-Constraint Sensitivity (CCS). Across 16 MLLMs, we find that imposing system messages substantially erodes base task accuracy, that compliance collapses under user conflict for open-weight models while remaining stable for top proprietary ones, and that vision-grounded constraints are the hardest category for every model.

==> tables/think_evaluation_2.tex <==
% \begin{table*}[t]
% \centering
% \caption{\textbf{Think! Constraint Satisfaction Rate(CSR) by Category.} 
% }
% % \vspace{0.3em}
% % \centering
% % \caption{Clustering}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccccccc}
% \toprule
% & & \multicolumn{2}{c}{\textbf{Format}} & \multicolumn{2}{c}{\textbf{Style}} & \multicolumn{2}{c}{\textbf{Background}} & \multicolumn{2}{c}{\textbf{Content}} & \multicolumn{2}{c}{\textbf{Visual}} & \multicolumn{2}{c}{\textbf{Total}} \\
% \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14} 
% \textbf{Model} & \textbf{Think} & AL & MA & AL & MA & AL & MA & AL & MA & AL & MA & AL & MA \\ 
% \midrule
% \midrule
% GPT-5.4-Mini~\citep{model_gpt5} & $\xmark$ & 86.3 & 83.1 & 73.6 & 60.8 & 70.9 & 66.6 & 83.0 & 74.2 & 64.5 & 52.5 & 75.7 & 67.4 \\
% GPT-5.4-Mini~\citep{model_gpt5} & $\checkmark$ & 89.5 & 87.9 & 77.4 & 76.8 & 80.4 & 80.1 & 88.3 & 88.3 & 75.6 & 74.0 & 82.2 & 81.4 \\
% \midrule
% GPT-5.4~\citep{model_gpt5} & $\xmark$ & 90.5 & 88.1 & 78.5 & 80.0 & 82.9 & 85.2 & 86.8 & 85.0 & 78.3 & 77.8 & 83.4 & 83.2 \\
% GPT-5.4~\citep{model_gpt5} & $\checkmark$ & 89.5 & 89.9 & 83.5 & 84.2 & 84.9 & 85.7 & 88.5 & 88.3 & 80.8 & 84.6 & 85.5 & 86.6 \\
% \midrule
% Claude-Sonnet-4.6~\citep{model_claude4} & $\xmark$ & 78.4 & 80.0 & 71.3 & 65.8 & 65.3 & 54.3 & 78.6 & 77.3 & 65.2 & 55.7 & 71.8 & 66.6 \\
% Claude-Sonnet-4.6~\citep{model_claude4} & $\checkmark$ & 78.2 & 77.2 & 70.9 & 68.6 & 68.4 & 57.7 & 78.2 & 74.7 & 63.6 & 53.4 & 71.8 & 66.3 \\
% \midrule
% Claude-Opus-4.7~\citep{model_claude4} & $\xmark$ & 84.5 & 82.5 & 78.1 & 77.6 & 78.6 & 68.6 & 85.7 & 81.1 & 69.2 & 63.3 & 79.2 & 74.6 \\
% Claude-Opus-4.7~\citep{model_claude4} & $\checkmark$ & 87.9 & 81.0 & 77.6 & 74.5 & 77.0 & 66.3 & 84.8 & 79.5 & 65.4 & 59.0 & 78.6 & 72.1 \\
% \bottomrule
% % \vspace{-0.5em}
% \end{tabular}
% }
% \label{table:think_mode_csr}
% \end{table*}

\begin{table*}[t]
\centering
\caption{\textbf{Think! Joint Satisfaction Rate(JSR) by Category.} 
}
% \vspace{0.3em}
% \centering
% \caption{Clustering}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
\toprule
& & \multicolumn{2}{c}{\textbf{Format}} & \multicolumn{2}{c}{\textbf{Style}} & \multicolumn{2}{c}{\textbf{Background}} & \multicolumn{2}{c}{\textbf{Content}} & \multicolumn{2}{c}{\textbf{Visual}} & \multicolumn{2}{c}{\textbf{Total}} \\
\cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14} 
\textbf{Model} & \textbf{Think} & AL & MA & AL & MA & AL & MA & AL & MA & AL & MA & AL & MA \\ 
\midrule
\midrule
GPT-5.4-Mini~\citep{model_gpt5} & $\xmark$ & 38.2 & 26.5 & 33.5 & 22.0 & 31.0 & 24.2 & 36.2 & 24.2 & 26.5 & 18.9 & 33.3 & 23.2 \\
GPT-5.4-Mini~\citep{model_gpt5} & $\checkmark$ & 42.1 & 32.3 & 37.8 & 29.9 & 35.6 & 28.4 & 40.7 & 31.1 & 36.9 & 27.7 & 38.8 & 30.0 \\
\midrule
GPT-5.4~\citep{model_gpt5} & $\xmark$ & 43.2 & 35.2 & 40.2 & 33.8 & 38.9 & 29.7 & 41.5 & 32.4 & 40.0 & 25.6 & 40.9 & 31.5 \\
GPT-5.4~\citep{model_gpt5} & $\checkmark$ & 45.8 & 34.9 & 42.5 & 33.9 & 42.1 & 32.0 & 44.9 & 32.5 & 40.4 & 32.6 & 43.2 & 33.3 \\
\midrule
Claude-Sonnet-4.6~\citep{model_claude4} & $\xmark$ & 42.7 & 31.0 & 38.7 & 26.9 & 32.0 & 21.7 & 41.1 & 27.3 & 34.0 & 20.8 & 38.0 & 25.8 \\
Claude-Sonnet-4.6~\citep{model_claude4} & $\checkmark$ & 41.5 & 26.3 & 37.7 & 27.2 & 37.8 & 21.2 & 38.8 & 25.7 & 33.2 & 20.5 & 37.9 & 24.3 \\
\midrule
Claude-Opus-4.7~\citep{model_claude4} & $\xmark$ & 47.3 & 32.9 & 42.6 & 33.8 & 41.3 & 26.3 & 44.9 & 29.5 & 37.8 & 23.7 & 42.9 & 29.5 \\
Claude-Opus-4.7~\citep{model_claude4} & $\checkmark$ & 46.3 & 32.0 & 40.8 & 31.0 & 41.2 & 25.3 & 42.2 & 28.4 & 37.0 & 26.2 & 41.6 & 28.8 \\
\bottomrule
% \vspace{-0.5em}
\end{tabular}
}
\label{table:think_mode_csr}
\end{table*}
